Beyond I.I.D.: Three Levels of Generalization for Question Answering on Knowledge Bases

Existing studies on question answering on knowledge bases (KBQA) mainly operate with the standard i.i.d assumption, i.e., training distribution over questions is the same as the test distribution. However, i.i.d may be neither reasonably achievable nor desirable on large-scale KBs because 1) true user distribution is hard to capture and 2) randomly sample training examples from the enormous space would be highly data-inefficient. Instead, we suggest that KBQA models should have three levels of built-in generalization: i.i.d, compositional, and zero-shot. To facilitate the development of KBQA models with stronger generalization, we construct and release a new large-scale, high-quality dataset with 64,331 questions, GrailQA, and provide evaluation settings for all three levels of generalization. In addition, we propose a novel BERT-based KBQA model. The combination of our dataset and model enables us to thoroughly examine and demonstrate, for the first time, the key role of pre-trained contextual embeddings like BERT in the generalization of KBQA.

==> experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experiment Setup}

\noindent \textbf{Data split.}
We set up two evaluation settings. In the \textit{in-domain} setting, a parser is evaluated on domains it has seen in training but possibly with novel compositions. In the \textit{cross-domain} setting, a parser needs to generalize to unseen domains in a zero-shot fashion. The same training data is used for both settings. Statistics are shown in Table~\ref{table:split}. For the cross-domain setting, 10 domains are held out for dev and another 10 for test.

\begin{table}[]
    \small
    \centering
    \begin{tabular}{cccc} \toprule
        & \textbf{Train} & \textbf{Dev} &\textbf{Test} \\ \midrule
        \textbf{In-domain} &  38,102 & 6,398 & 6,398\\
        \textbf{Cross-domain}  & 38,102 & 6,756 & 6,962 \\
        \bottomrule
    \end{tabular}
    \caption{Data split.}
    \label{table:split}
    \vspace{-10pt}
\end{table}

\noindent \textbf{Evaluation metric.}
We use exact match accuracy, i.e., the percentage of questions where the predicted logical form and the gold logical form are semantically identical. To determine the semantic equivalence between two logical forms, we first convert logical forms into the graph-shaped meaning representation from~\citet{su-etal-2016-generating}, which reduces the problem to graph isomorphism recognition\footnote{\url{https://networkx.github.io}}. Unlike string-based or set-based exact match~\cite{yu-etal-2018-spider}, our graph isomorphism based exact match is both sound and complete in identifying equivalent formulas.
%We use two metrics for evaluation, i.e., exact match and F1. Exact match denotes whether the predicted logical form and the target logical form are identical or not. To determine the semantic equivalence between two logical forms, we first convert logical forms into corresponding graph queries, and then reduce the problem into graph isomorphism recognition. Different from the string-based exact match or the set-based exact match~\cite{yu-etal-2018-spider}, this semantic-aware exact match is sound and complete in identifying equivalent formulas. Sometimes solely relying on exact match for evalutation can be too strict, to be specific, a partially correct prediction should also be taken into account. So we also use F1 of the execution results as a metric because sometimes models are able to generate novel structure or get partially correct on the logical forms.

We fine-tune BERT and fix GloVe, because we find fine-tuning GloVe makes it worse. Other implementation details such as hyper-parameters and the training scheme can be found in Appendix~\ref{sec:appendix_setup}.
%For all models, we first use GloVe~\cite{pennington-etal-2014-glove} pretrained word embeddings to encode both the input utterance and schema items, and fix it during training. For each schema item, we represent it using the average word embeddings of its surface name. For ranking based models, we set the number of relations \textit{k} to be 2 since 3 relations will result in prohibitively many candidates.
%Besides, we also try to incorporate BERT~\cite{devlin-etal-2019-bert} into our model. We use the representations from BERT instead of GloVe for the BERT-based models as mentioned in Section.~\ref{bert-use}, and all other parts remain the same. Specifically, we only consider a subset of schema items\footnote{For every question, we use the schema items that meet the following two requirements: 1) falling into the same domains as the quesiton 2) can be reached within 2 hops by the topic entities} for each question during training. But this may still exceed BERT's maximum length limit, which is 512 tokens. So we divide the schema items into chunks with at most 50 schema items for each, then concatenate each chunk and the input utterance one-by-one. Last but not least, to address the challenge of identifying relevant schema items, we also add a \textbf{Vocabulary Pruning (VP)} component to reduce the search size of Seq2Seq model to schema items reachable within 2-hops by the topic entities for every question.

\subsection{Results}
% \begin{table*}[t]
% \small
% \begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}cccccccc}
% \toprule
%                  %& \multicolumn{4}{c}{Exact Match}               \\ \hline
%                  & \multicolumn{4}{c}{\textbf{Perfect Entity Linking}} & \multicolumn{4}{c}{\textbf{BERT Entity Linker}}               \\ \hline
%                  & \multicolumn{2}{c}{In-domain} & \multicolumn{2}{c}{Cross-domain} & \multicolumn{2}{c}{In-domain} & \multicolumn{2}{c}{Cross-domain}\\ \hline
%                  &\textbf{Dev} &\textbf{Test} &\textbf{Dev} &\textbf{Test} &\textbf{Dev} &\textbf{Test} &\textbf{Dev} &\textbf{Test} \\ \hline
% \multicolumn{1}{l}{\textbf{Seq2Seq}} & \\\hline
% \multicolumn{1}{r}{+GloVe}    &  &0.537                          & & 0.016 & & 0.257 & & 0.008       \\ 
% \multicolumn{1}{r}{+GloVe+VP} & 0.638&0.556                          &0.041 &0.032    & &0.239 & &0.007    \\ 
% \multicolumn{1}{r}{+BERT}     & &0.366                          & &0.154  & &0.222 & &0.090       \\ 
% \multicolumn{1}{r}{+BERT+VP}  & 0.658&0.637                          &0.327 &0.326   & &\textbf{0.322} & &0.177     \\\hline
% \multicolumn{1}{l}{\textbf{Ranking}} & \\\hline
% \multicolumn{1}{r}{+GloVe}    & 0.655&\textbf{0.661}                          & 0.440&0.345   & &0.321 & &0.164     \\
% \multicolumn{1}{r}{+BERT}     &0.650 &0.657                          &0.567 &\textbf{0.585}       & &0.318 & &\textbf{0.303} \\ \bottomrule
% \end{tabular*}
% \caption{Overall results.}
% \label{table:overall}
% \vspace{-10pt}
% \end{table*}

\begin{table*}[t]
\small
\begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}cccc}
\toprule
                 %& \multicolumn{4}{c}{Exact Match}               \\ \hline
                 & \multicolumn{2}{c}{\textbf{Perfect Entity Linking}} & \multicolumn{2}{c}{\textbf{BERT Entity Linker}}               \\ \hline
                 & In-domain & Cross-domain & In-domain & Cross-domain\\ \hline
\multicolumn{1}{l}{\textbf{Seq2Seq}} & \\\hline
\multicolumn{1}{r}{+GloVe}    &0.537                          &0.016 & 0.257 & 0.008       \\ 
\multicolumn{1}{r}{+GloVe+VP} &0.556                        &0.032 &0.239 &0.007    \\ 
\multicolumn{1}{r}{+BERT}     &0.366                          &0.154  &0.222 &0.090       \\ 
\multicolumn{1}{r}{+BERT+VP}  &0.637                          &0.326   &\textbf{0.322} &0.177     \\\hline
\multicolumn{1}{l}{\textbf{Ranking}} & \\\hline
\multicolumn{1}{r}{+GloVe}   &\textbf{0.661}                        &0.345   &0.321 &0.164     \\
\multicolumn{1}{r}{+BERT}     &0.657                 &\textbf{0.585}       &0.318 &\textbf{0.303} \\ \bottomrule
\end{tabular*}
\caption{Overall results.}
\label{table:overall}
\vspace{-10pt}
\end{table*}


% \begin{table}[t]
% \caption{Overall results with BERT-based entity linking}
% \label{table:overall_el}
% \begin{tabular}{lcc}
% \toprule
%                  & \multicolumn{2}{c}{Exact Match}               \\ \hline
%                  & \multicolumn{1}{c}{Realistic} & Cross Domain \\ \hline
% Seq2Seq+GloVe    & 0.129                        &    0.002     \\ \hline
% Seq2Seq+GloVe+VP & 0.129                         &  0.003       \\ \hline
% Seq2Seq+BERT     & 0.126                          &0.072         \\ \hline
% Seq2Seq+BERT+VP  & 0.166                          & 0.111        \\ \hline
% Ranking+GloVe    & 0.167                         &  0.066       \\ \hline
% Ranking+BERT     & 0.173                         & 0.187        \\ \bottomrule
% \end{tabular}
% \end{table}
\subsubsection{Overall Evaluation}
%We present our experiment results here together with some insights drawn from the results. As depicted in table~\ref{table:cross}, for the cross-domain setting, the performances of two generation models, i.e., Seq2Seq and Grammar model, are both very low. Seq2Seq can only achieve an exact match of 5.2\%, while Grammar model is a little bit higher than Seq2Seq as it imposes constraints to guarantee well-formed logical forms during decoding. By comparison, Seq2Seq Ranking outperforms Seq2Seq significantly, which reveals the importance of taking account of the underlying structure of KB as prior knowledge. Note that, when incorporating BERT, the performance of Seq2Seq improves from 5.2\% to 37.1\%, and the performance of Seq2Seq Ranking improves from 48\% to 65.4\%. We argue that the reason for this is that BERT encodes much knowledge from the external corpus that can be transferable to any domain.
We show the overall results in Table~\ref{table:overall} with both perfect and BERT-based entity linker. All models perform significantly better in-domain than cross-domain, showing the challenge of zero-shot cross-domain generalization. Across all models, fine-tuned BERT brings a remarkable improvement, up to \textit{29\%}, over GloVe in the cross-domain setting. The trend may not be entirely surprising but the magnitude is. This strongly confirms the key role of pre-trained contextual embedding in cross-domain generalization. Ranking-based models generally outperform Seq2Seq models. We believe it can be attributed to that ranking-based models prune the search space more effectively by generating candidates based on topic entity's neighboring facts, while Seq2Seq models only use the schema. We also notice that the VP module plays an integral role in BERT-based models, even for the in-domain setting. A plausible reason is that when fine-tuning BERT-based models, we are only able to use a dynamic subset of the schema for each question, which lead to discrepancy between training and inference. The optimal way of using pre-trained contextual embeddings for OpenSP still remains to be investigated. 

%1. VP is more useful for cross-domain setting. This is because it is more challenging to identify the relevant schema items for cross-domain setting.

%2. Seq2Seq use the entire vocabulary for training while Seq2Seq + BERT only use a subset of vocabulary to train. This explains the performance on realistic setting, and also indicates the optimal way for using BERT in KBQA should be further studied.

%3. An interesting phenomenon we observed is that BERT can significantly improve the performance for cross-domain setting, but not the realistic setting.

%4. Ranking model performs much better than generation model, which reveals the importance of taking account of the underlying structure of KB.
 
\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/fine.pdf}
\caption{Fine-grained results.}
\label{fig:fine}
\end{figure}
\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{figs/equivalence.pdf}
\caption{Robustness analysis.}
\label{fig:para}
\vspace{-10pt}
\end{figure}

\subsubsection{Fine-grained Evaluation}
\label{sec:fine-grained}
We use perfect entity linking to reduce the number of variables in the fine-grained analysis\footnote{See results with BERT entity linker in Appendix~\ref{sec:appendix_fine}.}. We omit the vanilla Seq2Seq+BERT and Seq2Seq+GloVe baselines here for their subpar performance.

\noindent \textbf{Structural Complexity.} As shown in~\autoref{fig:fine}, the performance of all models degrades rapidly as questions become more compositional. Our ranking-based models are inherently unable to answer questions with more than 2 relations due to its exhaustive candidate generation. Seq2Seq models work better on compositional questions because they avoid exhaustive enumeration, though that comes with a penalty on simpler questions. Better guided search for both ranking and Seq2Seq generation may enjoy the best of both worlds. 

\noindent \textbf{Function.} Results on different functions are shown in~\autoref{fig:fine}. Note that ranking-based models rely on topic entities for candidate generation which are often absent in questions with comparatives or superlatives. Their performance suffers as a result. Comparatives and superlatives are also very challenging for Seq2Seq models, especially in the cross-domain setting. There is still a large room for improvement. 
%Specifically, some super questions have neither topic entity nor value (e.g., question \textit{what is the most distant nebula?}), which prevents the model from effectively reducing the search space. This type of question is also a unique feature in our dataset.

\noindent \textbf{Grounding \& Paraphrasing.} A good semantic parser should be robust to different paraphrases and groundings (e.g., succeed at \nl{Where is the Trump tower?} but fail at \nl{Where is the Tune Hotels?}). Our dataset provides an opportunity to directly test that. We create different groupings of questions: \emph{grouping by paraphrase} -- questions that are the same except for their entity groundings fall into the same group, and \emph{grouping by template} -- questions from the same logical form template (\autoref{fig:data_collection}) but have different groundings or paraphrases are grouped together.
Each grouping provides upper and lower bounds for evaluating model robustness. The upper bound is derived by treating all the questions in a group as correct if any of them is correctly answered, while the lower bound is derived by treating all the questions as incorrect if any of them is incorrectly answered. The true accuracy should lie between the bounds. The closer the three are, the more robust a model is to the corresponding mutation. The results are shown in Figure~\ref{fig:para}, which clearly show that  BERT-based models are generally more robust than GloVe-based models, which provides an explanation to its superior performance. Also, all models tend to be more sensitive to paraphrasing or grounding in cross-domain setting. 
%To show the robustness of different systems against paraphrasal questions, for each baseline, we rank all the paraphrases derived from the same graph query by their exact match achieved by the baseline, and then compute the average exact match of each rank. The results are illustrated in Figure~\ref{fig:para}. The robutness of a baseline can be described by the decreasing rate of a curve, i.e., the flatter the curve, the more robust the baseline. For both settings, ranking based models tend to be more robust than encoder-decoder models. Also, BERT based models perform relatively more stable than GloVe base models, which is kind of expected due to BERT's strong language modeling capability. \\

\noindent \textbf{Efficiency analysis.} We also report an efficiency analysis in Appendix~\ref{sec:appendix_efficiency}, which shows that, while ranking and VP bring significant accuracy gains, they also bring significant runtime overhead due to their search space pruning efforts.

%For the efficiency evaluation, we use online SPARQL exectution for both vocabulary pruning and candidate logical forms generation. Ranking based models run much slower than encode-decoder models, even when the maximal number of relations for candidate logical forms are restricted to be at most 2. Even ranking based models can achieve better accuracy, but its efficiency and scalability is questionable for practicality. 


% \begin{figure}[!h]
% \centering
% \includegraphics[width=\linewidth]{figs/time.pdf}
% \caption{Running time of different baselines.}
% \label{fig:time}
% \end{figure}

\subsection{Case Studies}
We illustrate several challenges in our dataset based on error analysis with BERT-based models.

\noindent \textbf{Exploiting KB for disambiguation. } 
%In the above results we show that ranking based models can significantly outperform the encoder-decoder models because they exploit the concrete facts in KB.\pl{isn't this more about incorporating type information, which isn't specific to ranking? you could have a decoder that only generated well-formed utterances, too right?} 
For question \nl{Flaminia brasini was the designer of what game?} that asks about \textrelation{games.game.designer}, Seq2seq models are confused by a similar relation \textrelation{computer.computer.key\_designers}. On the other hand, ranking-based model can more effectively reduce the large search space based on KB and predict the right formula as such a misleading relation would be eliminated during candidate generation.\\
%For the first question in Table~\ref{table:question}, the logical form predicated by Seq2Seq+BERT is \textrelation{(AND cvg.cvg\_platform (JOIN cvg.cvg\_platform.games Beats\_of\_Rage))}, which seems plausible. But in Freebase, \textentity{Beats\_of\_Rage} does not really have relation \textrelation{cvg.cvg\_platform.games}. On  the other hand, ranking based models generate candidate formulas from the KB, which means it will never encounter such a misleading formula, so it can properly predict the formula with correct relation \textrelation{cvg.cvg\_platform.games\_on\_this\_platform}.\\ 
%\textrelation{(AND cvg.cvg\_platform (JOIN cvg.cvg\_platform.games\_on\_this\_plat-\\form m.0kyq7h3))}. Open-schema semantic parsing always features a large search space, and we can greatly reduce the search space if we exploit the data in KB in a proper way. Generating candidate logical forms and then do ranking is the prevailing way to exploit KB data in literature, however, it always suffers from the flexibility to generalize to diverse query structures and the time efficiency.\\
\textbf{Ambiguity of expression. } A common challenge for OpenSP is that sometimes a relation may be expressed vaguely or ambiguously. For example, question \nl{Who produced the radio program on Paris?} is asking about the subject of a radio program. It involves an implicit relation \textrelation{radio.radio\_subject.programs\_with\_this\_subject}, while our model predicts \textrelation{broadcast.content.location}, which is asking about the location Paris. \\
%the corresponding logical form should be \textrelation{(AND cvg.computer\_game\_subject (JOIN cvg.computer\_game\_subject.games m.09v6kpg))}, while 
%the corresponding relation \textrelation{architecture.landscape\_architect.landscape\_project} is only expressed implicitly by \textit{created} in the question, while our model predicts a wrong relation \textrelation{architecture.architect.structures\_designed}.\\ 
%\textbf{Complex questions. } Complex questions that involve more than two relations can be extremely challenging to handle. For example, for question 3 with 3 relations in Table~\ref{table:question}, the model only predicted one relation and missed the other two. \\
%It is impractical to generate all the possible logical forms and then do ranking, so ranking based models fail on all those questions. Seq2Seq+BERT can occasionally get correct on some complex questions, but with an extremely low probability. 
%It is very challenging for the model to compose a complex formula that take into account all constraints. For question \textit{Which types of storage are compatible with Canon eos 650d as well as color filter array of bayer filter?}, the predicted formula is:\\\textrelation{(AND digicams.camera\_storage\_type (JOIN digicams.camera\_storage\_type.compatible\\\_cameras m.0j\_6g6y))}\\ 
%which only captures part of the correct formula by omitting another constraint on filter array type.\\
%which only captures part of the correct formula \\\textrelation{(AND digicams.camera\_storage\_type (AND (JOIN digicams.camera\_storage\_type.\\compatible\_cameras m.0j\_6g6y) \\(JOIN (R digicams.digital\_camera.\\supported\_storage\_types) (JOIN digicams.digital\_camera.color\\\_filter\_array\_type m.02r8js))))}.\\
%\textbf{Questions with no entity. } Ranking based models rely on topic entities to generate candidate logical forms, however, not all questions in our dataset have a topic entity. For instance, question 4 in Table~\ref{table:question} 
%has corresponding logical form \textrelation{(ARGMIN chemistry.chemical\_element chemistry.chemical\_element.discovery\_date)} with no entity in it.
%doesn't really involve a topic entity. This question can be correctly answered by encoder-decoder models while unable to be handled by ranking based models.\\
\textbf{Entity Linking Errors.} Entity disambiguation in previous datasets can always be simply done based on popularity, while in our dataset, many questions are not necessarily about popular entities. For \nl{Which Indonesian province's capital is Gorontalo?} our entity linker can identify the entity mention \textit{Gorontalo}, and the most popular entity has mention \textit{Gorontalo} is the province of Gorontalo, while the question is asking about the Gorontalo city. 
%To get a reasonable entity linking accuracy on our dataset, it is essential to take into account more contextual information from the questions.

\subsection{Transfer Learning}
\label{sec:transfer}

We also show that our dataset could serve as a valuable pre-training corpus for OpenSP in general by pre-training models on our dataset and fine-tuning on \WebQSP, which contains naturally-occurring questions from Google search log.
The results are shown in~\autoref{table:transfer}. We test three settings: Full training that fine-tunes using all training data of \WebQSP, few-shot that only uses 10\%, and zero-shot that directly applies models trained on our dataset to \WebQSP. We assume perfect entity linking. As shown in~\autoref{table:transfer} pre-trianing on our dataset uniformly improves the performance, especially in the low-data regime. Most remarkably, pre-trained on our dataset, the ranking model can achieve an F1 of 0.430 without any in-domain training on \WebQSP. These results also provide further evidence for the quality and diversity of our dataset.
%we first do pre-training on our dataset and then fine-tune on \WebQSP. Results in Table show that pre-training on our dataset can help to improve the performance on \WebQSP on both ranking and encoder-decoder setting.

\begin{table}[]
    \small
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule
     \multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{\textbf{Exact Match}}& \textbf{F1} \\ \midrule
    %  \textbf{Full Training} \\ \midrule
       \multirow{4}{*}{\textbf{Full Training}}&\textbf{s2s+BERT+VP}   &  0.42 & 0.46 \\
      &\multicolumn{1}{r}{+pre-training}   &  0.51 & 0.57 \\
      &\textbf{Ranking+BERT}     & 0.59 & 0.67\\
      &\multicolumn{1}{r}{+pre-training}   & \textbf{0.60} & \textbf{0.70} \\\midrule
    %   \textbf{Few-shot} \\ \midrule
     \multirow{4}{*}{\textbf{Few-shot}}& \textbf{s2s+BERT+VP}   & 0.21  &  0.31\\
      &\multicolumn{1}{r}{+pre-training}   &  0.34 & 0.47 \\
      &\textbf{Ranking+BERT}  & 0.44 & 0.53\\
      &\multicolumn{1}{r}{+pre-training} &\textbf{0.55} & \textbf{0.65}\\\midrule
    %   \textbf{Zero-shot}\\ \midrule
    \multirow{4}{*}{\textbf{Zero-shot}}& \textbf{s2s+BERT+VP}   & 0.00  &  0.00\\
      &\multicolumn{1}{r}{+pre-training}   &  0.14 & 0.20 \\
      &\textbf{Ranking+BERT}  & 0.00 & 0.00\\
      &\multicolumn{1}{r}{+pre-training} & \textbf{0.35} & \textbf{0.43}\\
      
    %  \multirow{2}{*}{\textbf{Zero-shot}}& \textbf{s2s+BERT+VP} & 0.14 & 0.20 \\
    %   &\textbf{Ranking+BERT} & \textbf{0.35} & \textbf{0.43} \\
    \bottomrule
    \end{tabular}}
    \caption{Transfer Learning Results on \WebQSP. "Pre-training" means pre-training on our dataset, and the base method is directly fine-tuning from BERT.}
    \label{table:transfer}
    \vspace{-10pt}
\end{table}


% \subsection{Limitations of Existing Methods}


% \begin{table*}[t]
% \caption{Results of Cross-domain Setting}
% \label{table:cross}
% \begin{tabular}{p{0.5\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}}
% \hline
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{\textbf{Exact Match}} & \textbf{F1} \\ \hline
% \textbf{Seq2Seq}                 &      0.331 0.009                                        &             \\ \hline
% \textbf{Seq2Seq + VP}                  &    0.359 0.029                                       &             \\ \hline
% % \multicolumn{1}{r|}{Perfect EL + Perfect DI} & \multicolumn{1}{l|}{0.050 0.371}                     &             \\
% % \multicolumn{1}{r|}{Perfect EL}              & \multicolumn{1}{l|}{0.029 (no DI) 0.359}                     &             \\
% % \multicolumn{1}{r|}{Realistic}               & \multicolumn{1}{l|}{}                     &             \\ \hline
% \textbf{Seq2Seq + BERT}           &     0.213 0.064                                      &             \\ \hline
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{0.291 0.559}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\ \hline
% \textbf{Seq2Seq + BERT + VP}           &    0.364 0.223                                       &             \\ \hline
% \textbf{Seq2Seq Ranking}                     &         0.612 0.462                                  &             \\ \hline
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{0.462 0.612}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\ \hline
% \textbf{Seq2Seq Ranking + BERT}              &     0.713 0.618                                      &             \\ \hline
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{0.618 0.713}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% % \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\ \hline
% \textbf{Grammar model}                  &                                           &             \\ \hline
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{0.089}                     &             \\
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\ \hline
% \textbf{Grammar Generation + BERT}           &                                           &             \\ \hline
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\
% \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                     &             \\ \hline
% \end{tabular}
% \end{table*}

==> unnecessary_template_files/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

